Holmes: A Benchmark to Assess the Linguistic Competence of Language Models

We introduce Holmes, a new benchmark designed to assess language models (LMs) linguistic competence - their unconscious understanding of linguistic phenomena. Specifically, we use classifier-based probing to examine LMs' internal representations regarding distinct linguistic phenomena (e.g., part-of-speech tagging). As a result, we meet recent calls to disentangle LMs' linguistic competence from other cognitive abilities, such as following instructions in prompting-based evaluations. Composing Holmes, we review over 270 probing studies and include more than 200 datasets to assess syntax, morphology, semantics, reasoning, and discourse phenomena. Analyzing over 50 LMs reveals that, aligned with known trends, their linguistic competence correlates with model size. However, surprisingly, model architecture and instruction tuning also significantly influence performance, particularly in morphology and syntax. Finally, we propose FlashHolmes, a streamlined version that reduces the computation load while maintaining high-ranking precision.

==> parts/7-Limitations-TACL.tex <==

\section*{Ethical Considerations and Limitations}
\Holmes{} as well as \FlashHolmes{} solely assess linguistic phenomena for the English language. 
Further, we agree with \citet{liang2023holistic} and perceive \Holmes{} as an incomplete snapshot of existing resources at a given time.   
Finally, as \Holmes{} relies on existing resources, it inherits existing bias, such as gender equality or underrepresentation of gender fairness, like the use of neo pronouns such as \textit{em} in \citet{lauscher-etal-2023-em}.


\section*{Acknowledgments}
We thank Yongxin Huang, Tim Baumgärtner, Ji-Ung Lee, the action editor, and anonymous reviewers for their valuable feedback and discussions.
Andreas Waldis is supported by the Hasler Foundation Grant No. 21024.

==> parts/x-colab-on-going.tex <==
\section{Collaboration}

\subsection{On-Going}


\subsubsection{Analysis of 2nd version of benchmark}

\begin{itemize}
    \item 202 tasks
    \item 43 LMs
    \item categorization according to linguistic capability, linguistic phenomena, probe type
    \item F1 score for classification tasks, person correlation for regression
\end{itemize}


\subsubsection{What could we remove?}

As in Figure 3 of the Flash-HELM paper, can/should we safely remove one specific:

\begin{itemize}
    \item \textit{Linguistic Subfield} like \textit{syntax}
    \item \textit{Probing Task Type} like \textit{span classification}
    \item \textit{Linguistic Phenomena} like \textit{part-of-speech}
    \item \textit{Probing Dataset} like \textit{xpos}
\end{itemize}

Rather a sanity check, we (hopefully) find ground to say we do not consider removing a whole \textit{Linguistic Subfield} because they all attribute to the final model ranking differently. 

\subsubsection{How much test data can we remove?}

\begin{itemize}
    \item trend analysis aggregated across all probing datasets (as in Figure 5 of the Flash-HELM paper)
\end{itemize}

\subsubsection{How much training data can we remove?}

\begin{itemize}
    \item trend analysis aggregated across all probing datasets (as in Figure 5 of the Flash-HELM paper)
\end{itemize}


\subsubsection{Generation of an efficient version}

The following pipeline would not require new experiments apart from the final efficient version of \Holmes
\begin{enumerate}
    \item Removal of redundant test instances per probing datasets individually (reduce encoding time, which dominates probing time for large LMs and datasets)
    \item Removal of redundant probing datasets
    \item Removal of training instances per probing dataset individually
\end{enumerate}




==> parts/y-colab-backlog.tex <==

\subsection{Backlog}


\subsubsection{Are different metrics necessary?}
\begin{itemize}
    \item F1, accuracy, pearson correlation
    \item Compression based on the minimum description length, how much data does a probe compress, \textbf{expensive to compute}
    \item Selectivity, how much worse does a probe perform when we train with randomly shuffled labels, we do not want that a probe learns much but rather detection the existence of a pattern, \textbf{expensive to compute}
\end{itemize}

\subsubsection{Number of intermediate layers in the probe?}
\begin{itemize}
    \item Having one or two hidden layers
\end{itemize}

\subsubsection{How can we select tasks?}
\begin{itemize}
    \item Difficulty
    \item Discriminability
    \item Task-task correlation (screenshot discussed during meeting)
\end{itemize}


\subsubsection{How well does an efficient benchmark derived with training LMs generalize to testing LMs?}
\begin{itemize}
    \item Which LMs to take for the training set?
    \item Randomly, cross-validated
    \item Task-task correlation (screenshot discussed during meeting)
\end{itemize}



\subsubsection{Is it meaningful to derive multiple versions of efficient benchmark regarding different scenarios?}
\begin{itemize}
    \item Model family (enc-only, dec-only, enc-dec)
    \item Pre-trained vs. instruction/chat fine-tuned
\end{itemize}



==> parts/z-colab-done.tex <==

\subsection{Done}

==> parts/z_1-Introduction.old.tex <==
\section{Introduction Old}
\label{sec:introduction}
% it seems like LM have good linguistic knowledge, but it requires verification
Language models (LMs) have seemingly demonstrated strong \textit{linguistic knowledge}, but to which extent requires verification \citep{mahowald2023dissociating}.
They might only grasp language superficially and struggle with generalization \citep{mccoy-etal-2019-right}, or excel in some areas while failing in others, differing from human language patterns \citep{DBLP:journals/tacl/WarstadtPLMPWB20,choshen-etal-2022-grammar}.
To assess LMs' linguistic knowledge, researchers have developed probing tests using linear classifiers to predict linguistic phenomena from their embeddings \citep{belinkov-2022-probing}, like part-of-speech (POS) of words \citep{belinkov-etal-2017-neural,liu-etal-2019-linguistic}. 
When these probes successfully and reliably extract linguistic phenomena under test, it suggests that LMs possess knowledge about specific linguistic aspects \citep{voita-titov-2020-information, hewitt-liang-2019-designing}.

Other from established LM evaluation studies, recent works \citep{Hendrycks2020MeasuringMM,cobbe2021gsm8k,Srivastava2022BeyondTI} significantly understudy linguistic knowledge,
mainly assessing LMs through user-centered tasks and covering a narrow spectrum of linguistic phenomena.
Examples include part-of-speech or named entities \citet{blevins-etal-2023-prompting}, linguistic acceptance \citet{liang2023holistic}, and plausibility pretesting \citet{amouyal2024large}.
Apart from the limited linguistic scope, these works rely on in-context learning (ICL), an evaluation methodology depending heavily on the text instructions provided \citep{lu2023emergent}, leading to performance variability \citep{mizrahi2023state,weber-etal-2023-mind,voronov2024mind,sclar2023quantifying}.
Thus, unlike classifier-based probing, ICL does not provide the stability to verify linguistic knowledge precisely and enhance our understanding of LMs. 



%In this paper, we 
%Using such evaluations, we describe and compare LMs from a linguistic perspective considering different textual granularities: part-of-speech (POS) of words or their dependency \citep{Tenney2019WhatDY, hewitt-manning-2019-structural}, the tense of sentences \citep{conneau-etal-2018-cram}, or phenomena encompassing the broader context of language like discourse rhetoric structure \citep{koto-etal-2021-discourse} and argumentation \citep{slonim2021autonomous}.

This paper introduces \Holmes{} (\autoref{fig:overview_Holmes{}}), a comprehensive benchmark for evaluating linguistic knowledge in language models (LMs) through classifier-based probing. \Holmes{} examines various linguistic aspects, including part-of-speech (POS), sentence tense, and discourse structure, among others, to understand LMs' capabilities and limitations more deeply.

This paper expands the scope of LM evaluation to the field of linguistics.
These capabilities are fundamental to understanding LMs' strengths and limitations as we continuously rely on text to interact with them.  
Therefore, we propose \Holmes{} (\autoref{fig:overview_Holmes{}}), the most comprehensive LM evaluation benchmark that precisely \underline{\textit{investigates}} linguistic knowledge in the \textbf{representations} of LMs.% based on classifier-based probing.
\Holmes{} considers textual granularities from single words (like POS) to the broader context of language like discourse rhetoric structure \citep{koto-etal-2021-discourse}.
More precisely, \Holmes{} contains the following components:

\paragraph{Meta-Analysis (\autoref{sec:survey})}
We review 274 probing studies from 2018 to 2023, focusing on linguistic knowledge of LMs. 
We systematically extract probing methodology and covered tasks and LMs.
We found a majority (75\%) of these studies using classifier-based probing, addressing over 200 tasks and 150 LMs.
Despite this broad scope, we identified significant gaps: only three LMs were tested on more than 20\% of the tasks, just one task was evaluated across more than 20\% of the LMs, and latest larger LMs are completely absent.


\paragraph{Benchmark (\autoref{sec:holmes})}
With \Holmes{}, we form a comprehensive ground to fill this identified blind spot.
Specifically, we consolidate existing resources and form 202 distinct \textit{probing datasets} verifying 74 \textit{linguistic phenomena}.
We group these phenomena into five linguistic competencies: \emph{morphology}, \emph{syntax}, \emph{semantics}, \emph{reasoning}, and \emph{discourse}.   

\paragraph{Evaluation and Analysis (\autoref{sec:full})}
These experiments confirm its meaningfulness and significance as \Holmes{} comprehensively fills the blind and manifold spot of linguistic knowledge in the LM evaluation landscape.
Aligned with other downstream competencies, verified in \textit{OpenLLM} \citep{Pham_OpenLLM_Operating_LLMs_2023} \Holmes{} provides a unique and supplementary perspective to understand LMs.  
In general, no single language model consistently outperforms the others across all tasks.
Instead, we found model architecture, size, and instruction fine-tuning strongly influence different linguistic strengths of LMs (\autoref{fig:findings}). 

\paragraph{Efficiency (\autoref{sec:efficient})}
Finally, we acknowledge the heavy computational burden of evaluating a \textbf{new} LM on \Holmes{}.
We form the streamlined version \FlashHolmes{} by selectively excluding probing datasets and samples that do not significantly influence the overall LM rankings \citep{rodriguez-etal-2021-evaluation, perlitz2023efficient}.
It approximates \Holmes{} saving a sixteenth of the computational costs while offering high precision.
\begin{comment}


\end{comment}
\begin{figure}[t]
%\footnotesize
	\begin{minipage}{0.48\textwidth}
    \begin{mybox}
    \textbf{i)} LMs internally strongly encode formal linguistic competencies (i.e., \textit{syntax}), but rather lack functional ones like \textit{reasoning}.\\
    \textbf{ii)} Linguistic competencies of pre-trained LMs scale after having 500 million parameters.\\
    \textbf{iii)} Instruction fine-tuning further enhances linguistic knowledge, especially for large LMs.\\
    \textbf{v)} Model architecture crucially influences what linguistic competencies LMs grasp.
    We found that token representations of decoder-only LMs lack stability which is resolved when scaling the LMs to 12 billion or more.\\
    \end{mybox}
    \end{minipage}
    \caption{Key evaluation finding of \Holmes{}.}
    \label{fig:findings}
\end{figure}


\paragraph{Contributions}
% Summing up,
This work sheds light on the meaningfulness of comprehensively verifying linguistic knowledge of LMs in their representations, 
%a previous blind spot in current LM evaluation: 
addressing a previously overlooked aspect of LM evaluation and enriching our understanding of their linguistic capabilities. Below we summarize the key contributions of our work: 

\textbf{1)} We present \Holmes{} marking the up-to-date, most comprehensive systematic review and consolidated collection of resources to verify the multiplicity of linguistic knowledge encoded in LMs.

\textbf{2)} We exhaustively experiment with 50 diverse LMs to tackle the gap in understanding their linguistic knowledge. %address the lack of knowledge about their linguistic knowledge.
Numerous insights and the supplementary nature of \Holmes{} to other LM evaluation benchmarks underscore its significance for LM evaluation. 

\textbf{3)} We form a streamlined version \FlashHolmes{} allowing to efficiently approximate rankings of new upcoming LMs.

\textbf{4)} We foster methodological and empirical progress by releasing detailed results and evaluation code. 

